Holographic BCFT Spectra from Brane Mergers

We use holography to study the spectra of boundary conformal field theories (BCFTs). To do so, we consider a 2-dimensional Euclidean BCFT with two circular boundaries that correspond to dynamical end-of-the-world branes in 3-dimensional gravity. Interactions between these branes inform the operator content and the energy spectrum of the dual BCFT. As a proof of concept, we first consider two highly separated branes whose only interaction is taken to be mediated by a scalar field. The holographic computation of the scalar-mediated exchange reproduces a light scalar primary and its global descendants in the closed-string channel of the dual BCFT. We then consider a gravity model with point particles. Here, the interaction of two separated branes corresponds to a heavy operator which lies below the black hole threshold. However, we may also consider branes at finite separation that "merge" non-smoothly. Such brane mergers can be used to describe unitary sub-threshold boundary-condition-changing operators in the open-string spectrum of the BCFT. We also find a new class of sub-threshold Euclidean bra-ket wormhole saddles with a factorization puzzle for closed-string amplitudes.

==> figs/Merging_strips_multiple.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\node[inner sep=0pt] (img) at (0,0)
    {\includegraphics{figs/merging_strip_branes_equal_many.pdf}};
\end{tikzpicture}
\caption{Intersecting strip branes.} 
\label{figs:manyintstrips}
\end{figure}

==> figs/Slicings_disks.tex <==
\begin{figure}[t]
\subfloat[\label{figs:diskslice}]
{\includegraphics{figs/disk_slicing.pdf}}
\hspace{1.5cm}
\subfloat[\label{figs:disksliceintpos}]
{\includegraphics{figs/disk_slicing_int_pos.pdf}}
\hspace{1.5cm}
\subfloat[\label{figs:disksliceintneg}]
{\includegraphics{figs/disk_slicing_int_neg.pdf}}
\caption{Slicings of disk brane configurations used in the computation of their Euclidean on-shell actions. We identify $u$ with the angular ($\phi$) direction in \eqref{conicalglobalads}. Note that the central $r = 0$ line (which is the position of the conical defect) is a horizon in this slicing.}
\label{figs:diskslices}
\end{figure}

==> figs/Slicings_strips.tex <==
\begin{figure}[t]
\subfloat[\label{figs:stripsliceneg}]
{\includegraphics{figs/strip_slicing_neg.pdf}}\hspace{2cm}
\subfloat[\label{figs:stripslicepos}]
{\includegraphics{figs/strip_slicing_pos.pdf}}
\caption{Slicings of annulus brane configurations used in the computation of their Euclidean on-shell actions. We identify $u$ with the angular ($\tau$) direction in \eqref{conicalglobalads}. In (b), the conical defect is integrated over in the slice, but it does not actually contribute to the on-shell action because it is orthogonal to each Cauchy slice.}
\label{figs:stripslice}
\end{figure}

==> figs/Wrapping_strip_branes.tex <==
\begin{figure}[t]
\centering
\includegraphics{figs/strip_branes.pdf}
\caption{Cross sections of $|T| = 1/2$ strip branes for decreasing values of $\alpha$. For $\alpha = 1$, the brane's endpoints are antipodal. For $\alpha < 1\slash 2$, the brane self-intersects in the bulk.} 
\label{figs:wrappingstrips}
\end{figure}

==> figs/adsFoliationSpherical.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\draw[-] (-2.5,0) to (2.5,0);
%\draw[-] (0,0) to (0,4);

\draw[-,red,thick,dashed] (1,0) arc (-60:240:2);
\draw[-,red,thick,dashed] (1,0) arc (-45:225:1.414);
\draw[-,red,thick,dashed] (1,0) arc (-30:210:1.155);
\draw[-,red,thick,dashed] (1,0) arc (0:180:1);
\draw[-,red,thick,dashed] (1,0) arc (45:135:1.414);


\node[red] at (-1,0) {$\bullet$};
\node at (-1,0) {$\circ$};
\node[red] at (1,0) {$\bullet$};
\node at (1,0) {$\circ$};

\draw[->,very thick] (0,1.25) to (0,3);
\node at (0.3,3) {$\varphi$};

\draw[->,very thick] (2.3,1.8) arc (0:45:2.3);
\draw[->,very thick] (-2.3,1.8) arc (180:135:2.3);
\node at (2.3,3) {$w$};
\node at (-2.3,3) {$w$};

\draw[<->,very thick] (1,-0.3) to (-1,-0.3);
\node at (0,-0.6) {$2\alpha$};
\end{tikzpicture}
\caption{A representation of the spherical foliation of Euclidean AdS$_{d+1}$ labeled by $\alpha$. The $\varphi$ coordinate labels the different AdS$_d$ slices, starting at $0$ and ending at $\pi$. The $w$ coordinate increases from the conformal boundary along each slice, starting at $0$ and reaching $2\alpha$ at the ``middle" of each ball. The geometric interpretation of $\alpha$ as the (renormalized) radius of the $(d-1)$-spherical boundary of each AdS$_d$ slice is also shown.}
\label{figs:adsFoliationSpherical}
\end{figure}

==> figs/annulus_brane_examples.tex <==
\begin{figure}[t]
\subfloat[\label{figs:closebdy}]
{\includegraphics{figs/close_to_bdy.pdf}}
\hspace{2cm}
\subfloat[\label{figs:farbdy}]
{\includegraphics{figs/far_from_bdy.pdf}}
\caption{Two examples of intersecting annulus brane configurations. In (a) $\alpha = 0.95$, so the intersection is close to the conformal boundary and the configuration is almost like a single smooth brane. In (b) $\alpha = 0.2$, so the intersection point is close to the center. The configuration (a) is dual to a BCC operator with dimension $\Delta_{\text{bcc}} \approx 0$, and the configuration (b) is dual to $\Delta_{\text{bcc}} \approx \frac{c}{12}$.}
\label{figs:rstarcostheta}
\end{figure}

==> figs/disk_brane_confs.tex <==
\begin{figure}[t]
\subfloat[\label{figs:posdisconnected}]
{\includegraphics{figs/two_disk_branes_small.pdf}}
\hspace{1cm}
\subfloat[\label{figs:posintersecting}]
{\includegraphics{figs/two_pos_disk_branes_int.pdf}}
\hspace{1cm}
\subfloat[\label{figs:negdisconnected}]
{\includegraphics{figs/two_disk_branes_small_neg.pdf}}
\hspace{1cm}
\subfloat[\label{figs:negintersecting}]
{\includegraphics{figs/two_disk_branes_small_neg_int.pdf}}
\caption{Four types of disk-brane configurations studied in this paper: (a) disconnected positive-tension branes, (b) intersecting positive-tension branes obtained by cutting and gluing along the dashed black lines, (c) disconnected negative-tension branes, and (d) intersecting negative-tension branes.}
\label{figs:diskbraneconfs}
\end{figure}

==> figs/intersecting_annulus_branes.tex <==
\begin{figure}[t]
\subfloat[\label{figs:rotstripbranes}]
{\includegraphics{figs/rotated_strip_branes.pdf}}\qquad
\subfloat[\label{figs:intstripbranes}]
{\includegraphics{figs/merging_strip_branes.pdf}}
\qquad
\subfloat[\label{figs:rotstripbranesneg}]
{\includegraphics{figs/rotated_strip_branes_negative.pdf}}
\qquad
\subfloat[\label{figs:intstripbranesneg}]
{\includegraphics{figs/merging_strip_branes_negative.pdf}}
\caption{Intersecting annulus brane configurations obtained from taking two different strip branes at $\alpha = \frac{2}{3} < 1$ and rotating them with respect to each other. By taking particular legs of the individual branes that meet at a single intersection point, we get (b) from (a) and (d) from (c).}
\label{figs:intstripbraneconf1}
\end{figure}
